The TESS Grand Unified Hot Jupiter Survey. II. Twenty New Giant Planets

NASA's Transiting Exoplanet Survey Satellite (TESS) mission promises to improve our understanding of hot Jupiters by providing an all-sky, magnitude-limited sample of transiting hot Jupiters suitable for population studies. Assembling such a sample requires confirming hundreds of planet candidates with additional follow-up observations. Here, we present twenty hot Jupiters that were detected using TESS data and confirmed to be planets through photometric, spectroscopic, and imaging observations coordinated by the TESS Follow-up Observing Program (TFOP). These twenty planets have orbital periods shorter than 7 days and orbit relatively bright FGK stars ($10.9 < G < 13.0$). Most of the planets are comparable in mass to Jupiter, although there are four planets with masses less than that of Saturn. TOI-3976 b, the longest period planet in our sample ($P = 6.6$ days), may be on a moderately eccentric orbit ($e = 0.18\pm0.06$), while observations of the other targets are consistent with them being on circular orbits. We measured the projected stellar obliquity of TOI-1937A b, a hot Jupiter on a 22.4 hour orbit with the Rossiter-McLaughlin effect, finding the planet's orbit to be well-aligned with the stellar spin axis ($|\lambda| = 4.0\pm3.5^\circ$). We also investigated the possibility that TOI-1937 is a member of the NGC 2516 open cluster, but ultimately found the evidence for cluster membership to be ambiguous. These objects are part of a larger effort to build a complete sample of hot Jupiters to be used for future demographic and detailed characterization work.

==> rv_data.tex <==
% target, bjdtdb, rv, rverr, bis, bis_err, inst
1937 & 2458883.646597 & -391.3 & 11.5 & 14 & 369 & PFS \\
1937 & 2458883.654039 & -315.0 & 10.7 & 117 & 370 & PFS \\
1937 & 2458885.696435 & 0.0 & 10.2 & 79 & 309 & PFS \\
1937 & 2458890.605451 & 283.1 & 8.8 & -70 & 194 & PFS \\
1937 & 2458915.545856 & -176.7 & 7.6 & 265 & 382 & PFS \\
1937 & 2458916.546030 & -285.4 & 8.7 & -13 & 503 & PFS \\
1937 & 2458921.623993 & -168.1 & 8.2 & -0 & 282 & PFS \\
1937 & 2458923.602326 & 58.7 & 9.1 & -114 & 269 & PFS \\
1937 & 2458925.540984 & 247.6 & 7.9 & 199 & 414 & PFS \\
1937 & 2459148.850625 & -182.4 & 8.5 & -67 & 236 & PFS \\
1937 & 2459149.853970 & 91.0 & 8.4 & 19 & 375 & PFS \\
1937 & 2459156.814317 & 149.4 & 7.4 & -306 & 90 & PFS \\
1937 & 2459157.782477 & 98.3 & 8.0 & -210 & 119 & PFS \\
2364 & 2459506.846343 & 21.2 & 3.4 & -68 & 40 & PFS \\
2364 & 2458109.760842 & -29.6 & 38.1 & -- & -- & TRES \\
2364 & 2458111.767217 & -36.6 & 31.6 & -- & -- & TRES \\
2364 & 2458552.719994 & -34.1 & 42.0 & -- & -- & TRES \\
2364 & 2458787.906462 & 0.0 & 38.1 & -- & -- & TRES \\
2364 & 2459531.768403 & 21.6 & 3.3 & 33 & 70 & PFS \\
2364 & 2459534.772396 & 0.0 & 2.9 & 37 & 34 & PFS \\
2364 & 2459592.689861 & -0.2 & 3.1 & 2 & 32 & PFS \\
2364 & 2459601.691493 & -35.0 & 3.2 & -33 & 36 & PFS \\
2364 & 2459602.728438 & -9.0 & 2.9 & -62 & 43 & PFS \\
2583 & 2459497.780143 & -22.7 & 6.7 & 32 & 43 & HIRES \\
2583 & 2459690.016743 & 21.8 & 5.8 & 10 & 36 & HIRES \\
2583 & 2459691.008175 & -5.2 & 6.0 & -10 & 38 & HIRES \\
2583 & 2459681.036672 & 15.6 & 6.7 & -59 & 57 & HIRES \\
2583 & 2459295.988643 & 17.4 & 44.5 & -- & -- & TRES \\
2583 & 2459741.976029 & -29.8 & 6.6 & 61 & 38 & HIRES \\
2583 & 2459302.930323 & 0.0 & 44.5 & -- & -- & TRES \\
2583 & 2459657.152635 & 17.1 & 6.4 & 14 & 44 & HIRES \\
2587 & 2459545.048827 & -24496.2 & 11.4 & -38 & 45 & NEID \\
2587 & 2459551.042893 & -24523.0 & 6.3 & -3 & 14 & NEID \\
2587 & 2459529.033763 & -24515.8 & 8.3 & -29 & 32 & NEID \\
2587 & 2459581.951522 & -24457.1 & 10.3 & 10 & 42 & NEID \\
2587 & 2459575.902477 & -24488.8 & 6.3 & 24 & 12 & NEID \\
2587 & 2459583.866063 & -24521.5 & 5.1 & 0 & 12 & NEID \\
2587 & 2459611.828776 & -24525.7 & 5.6 & -3 & 13 & NEID \\
2587 & 2459606.712729 & -24514.3 & 5.3 & 5 & 21 & NEID \\
2587 & 2459327.701424 & 0.0 & 35.9 & -- & -- & TRES \\
2587 & 2459341.654623 & 77.4 & 35.9 & -- & -- & TRES \\
2587 & 2459691.646110 & -24494.8 & 7.0 & 19 & 20 & NEID \\
2587 & 2459645.607526 & -24523.9 & 11.6 & -47 & 47 & NEID \\
2796 & 2459554.914346 & 20637.4 & 6.6 & -16 & 49 & NEID \\
2796 & 2459561.756113 & 20552.1 & 10.1 & 38 & 63 & NEID \\
2796 & 2459564.906237 & 20594.0 & 8.8 & -27 & 54 & NEID \\
2796 & 2459568.928010 & 20651.1 & 8.2 & -37 & 63 & NEID \\
2796 & 2459567.900558 & 20588.1 & 12.4 & -61 & 88 & NEID \\
2796 & 2459575.910820 & 20538.6 & 10.8 & 67 & 76 & NEID \\
2796 & 2459583.829068 & 20621.5 & 5.9 & 18 & 32 & NEID \\
2796 & 2459542.998762 & -35.6 & 5.5 & -- & -- & HIRES \\
2796 & 2459576.887066 & 4.2 & 5.5 & -- & -- & HIRES \\
2796 & 2459587.785483 & 30.2 & 5.4 & -- & -- & HIRES \\
2796 & 2459489.002194 & 120.8 & 48.9 & -- & -- & TRES \\
2796 & 2459501.009862 & 0.0 & 48.9 & -- & -- & TRES \\
2803 & 2459532.929975 & 365.0 & 87.8 & -- & -- & TRES \\
2803 & 2459595.769062 & 267.9 & 5.0 & 18 & 46 & PFS \\
2803 & 2459600.718681 & -33.8 & 6.4 & 18 & 56 & PFS \\
2803 & 2459592.698437 & -23.4 & 5.8 & 18 & 57 & PFS \\
2803 & 2459659.547674 & -23.4 & 5.5 & -48 & 43 & PFS \\
2803 & 2459529.967846 & 0.0 & 87.8 & -- & -- & TRES \\
2803 & 2459530.918626 & 507.7 & 84.0 & -- & -- & TRES \\
2803 & 2459653.547720 & 0.0 & 6.9 & -57 & 56 & PFS \\
2803 & 2459662.530081 & 256.0 & 6.2 & 22 & 178 & PFS \\
2818 & 2459622.562180 & 58920.0 & 27.0 & -41 & 39 & CHIRON \\
2818 & 2459569.724380 & 58907.0 & 30.0 & 14 & 182 & CHIRON \\
2818 & 2459571.761690 & 59038.0 & 30.0 & 49 & 159 & CHIRON \\
2818 & 2459597.754410 & 58868.0 & 27.0 & 19 & 215 & CHIRON \\
2818 & 2459595.759550 & 59071.0 & 23.0 & -32 & 191 & CHIRON \\
2818 & 2459620.570660 & 59093.0 & 33.0 & -0 & 35 & CHIRON \\
2818 & 2459653.586150 & 59081.0 & 24.0 & -47 & 28 & CHIRON \\
2842 & 2459521.015506 & 28.9 & 51.4 & -- & -- & TRES \\
2842 & 2459530.000445 & 0.0 & 51.4 & -- & -- & TRES \\
2842 & 2459602.760440 & -52.3 & 7.0 & -14 & 46 & PFS \\
2842 & 2459592.750984 & -19.4 & 6.3 & 1 & 42 & PFS \\
2842 & 2459654.550799 & 40.6 & 9.1 & 2 & 79 & PFS \\
2842 & 2459660.552604 & 0.0 & 5.4 & 54 & 43 & PFS \\
2842 & 2459600.729653 & 38.4 & 7.3 & 23 & 57 & PFS \\
2842 & 2459663.573079 & -29.7 & 6.6 & -88 & 52 & PFS \\
2977 & 2459666.612760 & 8013.0 & 37.0 & 26 & 52 & CHIRON \\
2977 & 2459716.503770 & 8076.0 & 29.0 & 55 & 82 & CHIRON \\
2977 & 2459662.558590 & 8054.0 & 31.0 & -40 & 46 & CHIRON \\
2977 & 2459677.543010 & 7578.0 & 27.0 & 3 & 65 & CHIRON \\
2977 & 2459717.503320 & 7567.0 & 36.0 & 16 & 66 & CHIRON \\
2977 & 2459722.453820 & 7592.0 & 57.0 & -28 & 62 & CHIRON \\
3023 & 2459750.483000 & -103.7 & 6.3 & -- & -- & PFS \\
3023 & 2459602.822488 & -110.7 & 4.8 & 3 & 38 & PFS \\
3023 & 2459600.838924 & 21.6 & 5.3 & -96 & 80 & PFS \\
3023 & 2459652.734549 & -69.5 & 4.5 & 82 & 67 & PFS \\
3023 & 2459654.714329 & 0.0 & 5.5 & 64 & 73 & PFS \\
3023 & 2459659.686296 & 22.5 & 4.6 & 114 & 98 & PFS \\
3364 & 2459592.832025 & -198.7 & 1.6 & 8 & 12 & PFS \\
3364 & 2459600.787384 & 71.2 & 2.2 & -2 & 25 & PFS \\
3364 & 2459652.694190 & 0.0 & 2.9 & 5 & 39 & PFS \\
3364 & 2459660.675521 & -31.5 & 2.6 & -6 & 31 & PFS \\
3364 & 2459658.700914 & 13.2 & 2.3 & -24 & 27 & PFS \\
3364 & 2459602.814167 & -181.0 & 2.4 & 5 & 27 & PFS \\
3688 & 2459546.905680 & -270.8 & 9.3 & 30 & 37 & NEID \\
3688 & 2459554.896326 & -55.6 & 9.8 & -34 & 33 & NEID \\
3688 & 2459561.851517 & -26.6 & 11.3 & -92 & 50 & NEID \\
3688 & 2459581.811652 & -86.0 & 14.4 & 108 & 86 & NEID \\
3688 & 2459568.669482 & -72.0 & 8.0 & 65 & 31 & NEID \\
3688 & 2459567.867476 & -68.6 & 16.7 & -11 & 104 & NEID \\
3688 & 2459589.668248 & -220.6 & 14.7 & -23 & 100 & NEID \\
3688 & 2459475.892341 & 0.0 & 47.9 & -- & -- & TRES \\
3688 & 2459496.829785 & 177.4 & 47.9 & -- & -- & TRES \\
3807 & 2459547.992443 & 0.0 & 31.2 & -- & -- & TRES \\
3807 & 2459557.960185 & -181.2 & 31.2 & -- & -- & TRES \\
3807 & 2459714.720560 & -28773.3 & 5.3 & 7 & 24 & NEID \\
3807 & 2459737.678737 & -28801.1 & 9.4 & 33 & 36 & NEID \\
3807 & 2459709.735091 & -28603.2 & 11.7 & -21 & 44 & NEID \\
3807 & 2459645.932438 & -28612.1 & 6.0 & -10 & 24 & NEID \\
3807 & 2459715.749781 & -28545.9 & 9.7 & -40 & 51 & NEID \\
3819 & 2459564.937403 & 30732.0 & 10.6 & -2 & 40 & NEID \\
3819 & 2459561.877073 & 30685.5 & 12.3 & -5 & 53 & NEID \\
3819 & 2459581.863297 & 30769.3 & 21.2 & -85 & 161 & NEID \\
3819 & 2459566.995347 & 30939.1 & 14.0 & -12 & 98 & NEID \\
3819 & 2459586.734583 & 30942.2 & 7.9 & 7 & 23 & NEID \\
3819 & 2459584.027644 & 30797.3 & 7.9 & 53 & 27 & NEID \\
3819 & 2459529.929340 & 0.0 & 39.0 & -- & -- & TRES \\
3819 & 2459537.926887 & -23.1 & 39.0 & -- & -- & TRES \\
3912 & 2459622.045864 & 0.0 & 33.8 & -- & -- & TRES \\
3912 & 2459626.907693 & 110.5 & 33.8 & -- & -- & TRES \\
3912 & 2459690.999642 & 1.0 & 5.5 & -64 & 77 & HIRES \\
3912 & 2459694.072190 & 40.7 & 6.4 & -93 & 86 & HIRES \\
3912 & 2459709.959643 & 6.8 & 5.6 & -8 & 91 & HIRES \\
3912 & 2459712.781939 & -49.3 & 5.7 & 5 & 68 & HIRES \\
3912 & 2459715.974641 & -20.0 & 5.7 & 0 & 36 & HIRES \\
3912 & 2459729.810120 & -38.7 & 6.2 & 58 & 72 & HIRES \\
3912 & 2459724.801982 & 57.6 & 5.8 & 74 & 37 & HIRES \\
3976 & 2459739.836858 & -11.6 & 5.7 & 37 & 40 & HIRES \\
3976 & 2459611.017390 & 0.0 & 32.0 & -- & -- & TRES \\
3976 & 2459627.013481 & -18.1 & 32.0 & -- & -- & TRES \\
3976 & 2459789.797188 & 5.7 & 6.0 & -- & -- & HIRES \\
3976 & 2459690.984737 & 12.6 & 6.1 & -10 & 95 & HIRES \\
3976 & 2459694.059436 & -9.3 & 6.4 & 14 & 49 & HIRES \\
3976 & 2459710.035155 & 12.8 & 6.0 & -55 & 49 & HIRES \\
3976 & 2459792.806700 & -12.7 & 6.1 & -- & -- & HIRES \\
3976 & 2459737.812146 & 12.1 & 5.9 & -22 & 40 & HIRES \\
3976 & 2459738.853383 & -7.4 & 6.0 & 18 & 40 & HIRES \\
3976 & 2459741.870226 & 5.9 & 6.2 & -22 & 41 & HIRES \\
3976 & 2459742.849822 & 31.3 & 6.4 & 67 & 43 & HIRES \\
3976 & 2459740.784396 & -0.4 & 5.9 & 1 & 45 & HIRES \\
3976 & 2459712.835924 & -26.5 & 6.1 & -68 & 40 & HIRES \\
4087 & 2459744.779833 & 383.2 & 45.8 & -- & -- & TRES \\
4087 & 2459715.734342 & -14364.8 & 15.6 & -86 & 112 & NEID \\
4087 & 2459617.002754 & -40.8 & 27.9 & -- & -- & TRES \\
4087 & 2459624.952450 & 175.6 & 31.3 & -- & -- & TRES \\
4087 & 2459714.711453 & -14265.7 & 7.8 & 25 & 24 & NEID \\
4087 & 2459716.791237 & -14208.8 & 9.2 & 33 & 29 & NEID \\
4087 & 2459738.805759 & 90.6 & 41.5 & -- & -- & TRES \\
4087 & 2459737.912830 & -14376.7 & 15.7 & 13 & 105 & NEID \\
4087 & 2459723.945741 & -14169.0 & 14.2 & -154 & 119 & NEID \\
4087 & 2459718.718122 & -14331.8 & 19.1 & -78 & 177 & NEID \\
4087 & 2459740.889534 & 0.0 & 34.7 & -- & -- & TRES \\
4087 & 2459741.796263 & 1512.7 & 164.6 & -- & -- & TRES \\
4087 & 2459742.791150 & 213.0 & 33.8 & -- & -- & TRES \\
4087 & 2459743.852507 & 175.5 & 34.7 & -- & -- & TRES \\
4087 & 2459708.979815 & -14319.2 & 12.3 & 16 & 53 & NEID \\
4145 & 2459546.911882 & 1901.9 & 5.2 & 17 & 15 & NEID \\
4145 & 2459551.896450 & 1863.6 & 5.6 & 17 & 21 & NEID \\
4145 & 2459568.893862 & 1782.3 & 8.2 & -55 & 37 & NEID \\
4145 & 2459567.876981 & 1834.2 & 10.9 & -107 & 77 & NEID \\
4145 & 2459561.866241 & 1835.8 & 8.9 & -34 & 51 & NEID \\
4145 & 2459564.924720 & 1767.0 & 11.3 & 127 & 123 & NEID \\
4145 & 2459479.861798 & 0.0 & 34.4 & -- & -- & TRES \\
4145 & 2459651.700911 & 1843.7 & 6.1 & -14 & 24 & NEID \\
4145 & 2459656.729383 & 1903.9 & 5.3 & 27 & 18 & NEID \\
4145 & 2459477.943585 & -11.6 & 34.4 & -- & -- & TRES \\
4463 & 2459645.983032 & -90370.5 & 3.9 & 8 & 12 & NEID \\
4463 & 2459473.720949 & 0.0 & 27.5 & -- & -- & TRES \\
4463 & 2459664.020088 & -90479.2 & 5.0 & 0 & 12 & NEID \\
4463 & 2459486.670830 & 262.9 & 27.5 & -- & -- & TRES \\
4463 & 2459679.003678 & -90394.4 & 3.9 & -2 & 9 & NEID \\
4463 & 2459700.942040 & -90425.7 & 3.8 & 0 & 11 & NEID \\
4463 & 2459728.916044 & -90264.5 & 3.9 & -3 & 14 & NEID \\
4463 & 2459731.963063 & -90285.1 & 3.1 & -8 & 9 & NEID \\
4791 & 2459658.510910 & 33533.0 & 59.0 & -119 & 74 & CHIRON \\
4791 & 2459654.560250 & 33628.0 & 28.0 & -24 & 86 & CHIRON \\
4791 & 2459589.846011 & 0.0 & 47.5 & -- & -- & TRES \\
4791 & 2459617.690654 & 398.7 & 47.5 & -- & -- & TRES \\
4791 & 2459656.534380 & 33958.0 & 48.0 & -50 & 160 & CHIRON \\
4791 & 2459660.570600 & 34019.0 & 44.0 & 20 & 70 & CHIRON \\
4791 & 2459662.514190 & 33582.0 & 59.0 & -127 & 85 & CHIRON \\
4791 & 2459664.510770 & 34045.0 & 56.0 & 85 & 127 & CHIRON \\

